Learning to Diversify for Product Question Generation

We address the product question generation task. For a given product description, our goal is to generate questions that reflect potential user information needs that are either missing or not well covered in the description. Moreover, we wish to cover diverse user information needs that may span a multitude of product types. To this end, we first show how the T5 pre-trained Transformer encoder-decoder model can be fine-tuned for the task. Yet, while the T5 generated questions have a reasonable quality compared to the state-of-the-art method for the task (KPCNet), many of such questions are still too general, resulting in a sub-optimal global question diversity. As an alternative, we propose a novel learning-to-diversify (LTD) fine-tuning approach that allows to enrich the language learned by the underlying Transformer model. Our empirical evaluation shows that, using our approach significantly improves the global diversity of the underlying Transformer model, while preserves, as much as possible, its generation relevance.

==> docs/00c5f20b-e676-419e-90e8-99affa0725f3 <==
{"id":"321241621323","lines":[{"id":"n0.3851416450923924","blocks":[],"style":{"align":"center"}},{"id":"n0.6616997253421777","blocks":[]},{"id":"n0.18502931681419943","blocks":[],"style":{"align":"center"}},{"id":"n0.6436592395458514","blocks":[{"id":"n0.026102479707263537","text":"\\diagram","type":"composite","elements":{"de7870956724590363":{"id":"de7870956724590363","lines":[{"id":"n0.3698239226344531","blocks":[{"id":"n0.5303523650957325","text":"shared weights"}]}],"shape":{"data":{"p":{"x":236.54400062561035,"y":298.2799999237061}},"anchor":"left-top","style":{"textColor":[208,2,27,1]}},"isTextMode":true,"isInGroup":false},"de12591983895612047":{"id":"de12591983895612047","lines":[{"id":"n0.14592059367365495","blocks":[{"id":"n0.7465192818642414","text":"Transformer "}],"style":{"align":"center"}},{"id":"n0.7925699400141755","blocks":[{"id":"n0.3270351209455873","text":"Decoder"}],"style":{"align":"center"}}],"shape":{"data":{"p":{"x":97.79998779296875,"y":216.79999542236328}},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de8430795961016215":{"id":"de8430795961016215","lines":[{"blocks":[{"text":"Transformer ","id":"n0.6943265936003351"}],"style":{"align":"center"},"id":"n0.6941375721479999"},{"blocks":[{"text":"Decoder","id":"n0.990902676037581"}],"style":{"align":"center"},"id":"n0.02220645999164672"}],"shape":{"data":{"p":{"x":378,"y":215}},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9495979570510391":{"id":"de9495979570510391","lines":[{"id":"n0.4315331130458082","blocks":[{"text":"question 1","id":"n0.5583812821294418"}]}],"shape":{"data":{"p":{"x":106.79998779296875,"y":259.7999954223633}},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de8793797222094755":{"id":"de8793797222094755","lines":[{"blocks":[{"text":"question 2","id":"n0.08141945717536148"}],"id":"n0.9700106745771637"}],"shape":{"data":{"p":{"x":392.5599868774414,"y":258.3999954223633}},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de15764215326072972":{"id":"de15764215326072972","lines":[{"blocks":[{"text":"Transformer ","id":"n0.1632910560519092"}],"style":{"align":"center"},"id":"n0.016427030294752232"},{"blocks":[{"id":"n0.10347454329340833","text":"Encoder"}],"style":{"align":"center"},"id":"n0.4461515774217919"}],"shape":{"data":{"p":{"x":241,"y":217}},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9578415436867911":{"id":"de9578415436867911","lines":[{"blocks":[{"text":"context","id":"n0.5776013621924494"}],"id":"n0.8921457567217299"}],"shape":{"data":{"p":{"x":260,"y":258.7999954223633}},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de058493116679863455":{"id":"de058493116679863455","lines":[{"id":"n0.7846105416736373","blocks":[{"id":"n0.696544731422206","text":"cosine loss"}]}],"shape":{"data":{"p":{"x":246.14400062561032,"y":133.07999992370605}},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de8348584391447416":{"id":"de8348584391447416","lines":[{"id":"n0.4681283488302155","blocks":[{"id":"n0.9313291247825797","text":"CD head"}]}],"shape":{"data":{"p":{"x":111.19999999999999,"y":174.07999992370605}},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de10736605535946286":{"id":"de10736605535946286","lines":[{"blocks":[{"text":"CD head","id":"n0.8671730626084257"}],"id":"n0.9075124094878446"}],"shape":{"data":{"p":{"x":396.4,"y":171.27999992370607}},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de19020855354933452":{"id":"de19020855354933452","lines":[{"blocks":[{"text":"CD loss","id":"n0.25171622460897103"}],"id":"n0.21619140141658644"}],"shape":{"data":{"p":{"x":117.54400062561035,"y":132.27999992370607}},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de38218656652902183":{"id":"de38218656652902183","lines":[{"blocks":[{"text":"CD loss","id":"n0.7216677081667626"}],"id":"n0.6965317273559095"}],"shape":{"data":{"p":{"x":403.94400062561033,"y":129.07999992370608}},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de7327981594306865":{"id":"de7327981594306865","lines":[{"blocks":[{"text":"\\overline","type":"composite","elements":{"value":{"lines":[{"blocks":[{"text":"h","id":"n0.7185976951620616"}],"id":"n0.716366881693842"}],"id":"n0.29129782786125435"}},"id":"n0.8328913917894016"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.2780232454516234","text":"1"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[],"id":"n0.6437175195126297"}],"id":"n0.3188199941533236"}},"id":"n0.6578725030227908"}],"id":"n0.03553686393472333"}],"id":"n0.7199331639558169"}},"id":"n0.9105142971431339"}],"id":"n0.3191496644230738"}],"shape":{"data":{"p":{"x":247.80000000000004,"y":157.0800018310547}},"anchor":"left-top"},"isMathDisplayMode":true,"isInGroup":false},"de7110946585701836":{"id":"de7110946585701836","lines":[{"blocks":[{"text":"\\overline","type":"composite","elements":{"value":{"lines":[{"blocks":[{"text":"h","id":"n0.33676155231536775"}],"id":"n0.9779892368049046"}],"id":"n0.893381867964276"}},"id":"n0.14530020659547005"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.1792745064382124","text":"2"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[],"id":"n0.11059105519701573"}],"id":"n0.3856051686678359"}},"id":"n0.6570068887069698"}],"id":"n0.695702902365005"}],"id":"n0.9320852703915636"}},"id":"n0.6040498395670992"}],"id":"n0.8047205738604599"}],"shape":{"data":{"p":{"x":304.20000000000005,"y":158.4800018310547}},"anchor":"left-top"},"isMathDisplayMode":true,"isInGroup":false}},"connections":[],"intersections":{"id":"di08192249514956096","items":[],"style":{}},"shapes":[{"id":"dp6614769431650531","type":"doc-rounded-rect","data":{"p1":{"x":370.79998779296875,"y":193},"p2":{"x":483.79998779296875,"y":258.8000030517578}},"style":{"fillColor":[155,155,155,0.24]}},{"id":"dp765300474202183","type":"doc-rounded-rect","data":{"p1":{"x":88.19998779296876,"y":194.79999542236328},"p2":{"x":202.19998779296876,"y":260.8000030517578}},"style":{"fillColor":[155,155,155,0.24]}},{"id":"dp9126281050905791","type":"rectangle","data":{"p1":{"x":386.1999877929687,"y":198.39999542236328},"p2":{"x":393.9999755859375,"y":207.39999542236328}},"style":{"fillColor":[236,233,197,1]}},{"id":"dp8837456171914766","type":"rectangle","data":{"p1":{"x":393.9999755859375,"y":198.39999542236328},"p2":{"x":401.7999633789062,"y":207.39999542236328}},"style":{"fillColor":[243,170,170,1]}},{"id":"dp16647876846132048","type":"rectangle","data":{"p1":{"x":401.7999633789062,"y":198.39999542236328},"p2":{"x":409.599951171875,"y":207.39999542236328}},"style":{"fillColor":[194,230,158,1]}},{"id":"dp2754073804862862","type":"rectangle","data":{"p1":{"x":409.599951171875,"y":198.39999542236328},"p2":{"x":417.3999389648437,"y":207.39999542236328}},"style":{"fillColor":[236,193,193,1]}},{"id":"dp38353729908878154","type":"rectangle","data":{"p1":{"x":417.3999389648437,"y":198.39999542236328},"p2":{"x":425.1999267578125,"y":207.39999542236328}},"style":{"fillColor":[223,95,95,1]}},{"id":"dp869779464802084","type":"rectangle","data":{"p1":{"x":425.1999267578125,"y":198.39999542236328},"p2":{"x":432.9999145507812,"y":207.39999542236328}},"style":{"fillColor":[215,221,91,1]}},{"id":"dp7766874406133824","type":"rectangle","data":{"p1":{"x":432.9999145507812,"y":198.39999542236328},"p2":{"x":440.79990234375,"y":207.39999542236328}},"style":{"fillColor":[213,240,185,1]}},{"id":"dp28192666932856736","type":"rectangle","data":{"p1":{"x":440.79990234375,"y":198.39999542236328},"p2":{"x":448.5998901367187,"y":207.39999542236328}},"style":{"fillColor":[248,233,233,1]}},{"id":"dp7103641308541404","type":"rectangle","data":{"p1":{"x":448.5998901367187,"y":198.39999542236328},"p2":{"x":456.3998779296875,"y":207.39999542236328}},"style":{"fillColor":[223,153,153,1]}},{"id":"dp36640532325503194","type":"rectangle","data":{"p1":{"x":456.3998779296875,"y":198.39999542236328},"p2":{"x":464.1998657226562,"y":207.39999542236328}},"style":{"fillColor":[248,231,28,1]}},{"id":"dp9269485498555605","type":"rectangle","data":{"p1":{"x":104.79998779296875,"y":199.79999542236328},"p2":{"x":112.5999755859375,"y":208.79999542236328}},"style":{"fillColor":[243,240,189,1]}},{"id":"dp17497129565627767","type":"rectangle","data":{"p1":{"x":112.5999755859375,"y":199.79999542236328},"p2":{"x":120.39996337890625,"y":208.79999542236328}},"style":{"fillColor":[206,187,55,1]}},{"id":"dp34787387798184555","type":"rectangle","data":{"p1":{"x":120.39996337890625,"y":199.79999542236328},"p2":{"x":128.199951171875,"y":208.79999542236328}},"style":{"fillColor":[217,231,58,1]}},{"id":"dp9097845093987313","type":"rectangle","data":{"p1":{"x":128.199951171875,"y":199.79999542236328},"p2":{"x":135.99993896484375,"y":208.79999542236328}},"style":{"fillColor":[230,189,123,1]}},{"id":"dp8148882842892533","type":"rectangle","data":{"p1":{"x":135.99993896484375,"y":199.79999542236328},"p2":{"x":143.7999267578125,"y":208.79999542236328}},"style":{"fillColor":[197,190,122,1]}},{"id":"dp3058869197077534","type":"rectangle","data":{"p1":{"x":145,"y":199.79999542236328},"p2":{"x":152.79998779296875,"y":208.79999542236328}},"style":{"fillColor":[212,218,144,1]}},{"id":"dp5639234849060932","type":"rectangle","data":{"p1":{"x":152.79998779296875,"y":199.79999542236328},"p2":{"x":160.5999755859375,"y":208.79999542236328}},"style":{"fillColor":[224,225,200,1]}},{"id":"dp17201780625853913","type":"rectangle","data":{"p1":{"x":160.5999755859375,"y":199.79999542236328},"p2":{"x":168.39996337890625,"y":208.79999542236328}},"style":{"fillColor":[248,231,28,1]}},{"id":"dp340067734641494","type":"rectangle","data":{"p1":{"x":168.39996337890625,"y":199.79999542236328},"p2":{"x":176.199951171875,"y":208.79999542236328}},"style":{"fillColor":[245,166,35,1]}},{"id":"dp9840231542170459","type":"rectangle","data":{"p1":{"x":176.199951171875,"y":199.79999542236328},"p2":{"x":183.99993896484375,"y":208.79999542236328}},"style":{"fillColor":[202,230,193,1]}},{"id":"dp9639956178987188","type":"doc-rounded-rect","data":{"p1":{"x":234.39998779296874,"y":195.79999542236328},"p2":{"x":337.3999877929688,"y":259.8000030517578}},"style":{"fillColor":[222,255,230,1]}},{"id":"dp37606888143376516","type":"rectangle","data":{"p1":{"x":248,"y":200.79999542236328},"p2":{"x":255.79998779296875,"y":209.79999542236328}},"style":{"fillColor":[184,233,134,1]}},{"id":"dp027512618117242926","type":"rectangle","data":{"p1":{"x":255.79998779296875,"y":200.79999542236328},"p2":{"x":263.5999755859375,"y":209.79999542236328}},"style":{"fillColor":[159,216,174,1]}},{"id":"dp37678850033279554","type":"rectangle","data":{"p1":{"x":263.5999755859375,"y":200.79999542236328},"p2":{"x":271.39996337890625,"y":209.79999542236328}},"style":{"fillColor":[127,173,230,1]}},{"id":"dp18055275514530034","type":"rectangle","data":{"p1":{"x":271.39996337890625,"y":200.79999542236328},"p2":{"x":279.199951171875,"y":209.79999542236328}},"style":{"fillColor":[201,217,223,1]}},{"id":"dp8106140502673234","type":"rectangle","data":{"p1":{"x":279.199951171875,"y":200.79999542236328},"p2":{"x":286.99993896484375,"y":209.79999542236328}},"style":{"fillColor":[174,225,223,1]}},{"id":"dp9354220697631588","type":"rectangle","data":{"p1":{"x":286.99993896484375,"y":200.79999542236328},"p2":{"x":294.7999267578125,"y":209.79999542236328}},"style":{"fillColor":[205,228,214,1]}},{"id":"dp7809636477006632","type":"rectangle","data":{"p1":{"x":296,"y":200.79999542236328},"p2":{"x":303.79998779296875,"y":209.79999542236328}},"style":{"fillColor":[57,122,194,1]}},{"id":"dp37355225870103403","type":"rectangle","data":{"p1":{"x":303.79998779296875,"y":200.79999542236328},"p2":{"x":311.5999755859375,"y":209.79999542236328}},"style":{"fillColor":[117,168,138,1]}},{"id":"dp14480516191834458","type":"rectangle","data":{"p1":{"x":311.5999755859375,"y":200.79999542236328},"p2":{"x":319.39996337890625,"y":209.79999542236328}},"style":{"fillColor":[149,175,95,1]}},{"id":"dp0265640600049879","type":"rectangle","data":{"p1":{"x":319.39996337890625,"y":200.79999542236328},"p2":{"x":327.199951171875,"y":209.79999542236328}},"style":{"fillColor":[87,194,187,1]}},{"id":"da9989576173951193","data":[{"x":327.199951171875,"y":209.79999542236328},{"x":370.79998779296875,"y":220.8000030517578}],"head":">","tail":"no","shaft":"-"},{"id":"da6120441434210948","data":[{"x":248,"y":209.79999542236328},{"x":203.79998779296875,"y":223.8000030517578}],"head":">","tail":"no","shaft":"-"},{"id":"dp4393411965244878","type":"doc-rounded-rect","data":{"p1":{"x":241.59999999999997,"y":133.07999992370605},"p2":{"x":326.79998779296875,"y":155.8000030517578}},"style":{"fillColor":[237,160,31,0.51]}},{"id":"da709510964088069","data":[{"x":184.2,"y":203.48000183105466},{"x":272.6,"y":182.68000183105468},{"x":272.2,"y":155.47999992370606}],"head":">","tail":"no","shaft":"-"},{"id":"da13856350194452882","data":[{"x":385.4,"y":202.28000183105468},{"x":299.40000000000003,"y":181.48000183105466},{"x":299.4,"y":156.28000183105468}],"head":">","tail":"no","shaft":"-"},{"id":"dp32573196558410844","type":"up-arrow","data":{"p1":{"x":87.39999999999999,"y":172.67999992370608},"p2":{"x":199,"y":192.67999992370605},"sizePercentage":0.2953020134228189},"style":{"fillColor":[167,187,211,1]}},{"id":"dp00644188455381367","type":"up-arrow","data":{"p1":{"x":373.79999999999995,"y":170.27999992370607},"p2":{"x":485.4,"y":190.27999992370604},"sizePercentage":0.2953020134228189},"style":{"fillColor":[167,187,211,1]}},{"id":"dp3196289553709024","type":"doc-rounded-rect","data":{"p1":{"x":113,"y":132.27999992370607},"p2":{"x":175.40000000000003,"y":155.00000305175783}},"style":{"fillColor":[245,166,35,0.51]}},{"id":"da3553068686748364","data":[{"x":143.2,"y":172.67999992370608},{"x":143.40000000000003,"y":154.67999992370605}],"head":">","tail":"no","shaft":"-"},{"id":"dp24796023422828717","type":"doc-rounded-rect","data":{"p1":{"x":399.4,"y":129.07999992370608},"p2":{"x":461.8,"y":151.8000030517578}},"style":{"fillColor":[245,166,35,0.51]}},{"id":"da20764068544841097","data":[{"x":429.59999999999997,"y":169.4799999237061},{"x":429.8,"y":151.47999992370603}],"head":">","tail":"no","shaft":"-"},{"id":"da7592563719622529","data":[{"p1":{"x":378.79998779296875,"y":254.8000030517578},"p2":{"x":360.29998779296875,"y":274.0250015258789},"cp":{"dx":-7,"dy":7},"cp2":{"dx":8.5,"dy":-10.224998474121094}},{"p1":{"x":360.29998779296875,"y":274.0250015258789},"p2":{"x":291.79998779296875,"y":301},"cp":{"dx":-16.5,"dy":12.424999237060547},"cp2":{"dx":26.5,"dy":-0.5}},{"p1":{"x":291.79998779296875,"y":301},"p2":{"x":195.79998779296875,"y":259},"cp":{"dx":-34,"dy":2.8000030517578125},"cp2":{"dx":5,"dy":23}}],"head":"f>","tail":"f<","shaft":"--","type":"cubic","settings":{"isControlPointBreak":true},"style":{"strokeColor":[208,2,27,1]},"headScale":1.4}],"settings":{"grid":true,"diagramHeight":448}}]},{"id":"n0.7341516807922368","blocks":[],"style":{"align":"center"}}],"pageSettings":{"pageSize":{"width":700}},"delayRenderCache":{"av":776,"map":{}},"___version":2,"version":2,"av":776}

==> eval_prev.tex <==
\section{Evaluation}\label{sec:eval}
\subsection{Experimental Setup}
\subsubsection{Datasets}
\subsubsection{Implementation and Training}
We use DBS~\cite{Vijayakumar2016DiverseBS}
\subsubsection{Baselines}
\begin{itemize}
    \item MLE (vanila seq2seq)
    \item hMup~\cite{shen2019mixture} (mixture-model for MT)
    \item KPCNet~\cite{Zhang-KPCNet} (seq2seq with attention and keyword selection + manual filtering)
    %\item GAN-Utility~\cite{rao-daume-iii-2019-answer}
    %\item GPT-2~\cite{radford2019-gpt2} (decoder-only)
    \item BART~\cite{lewis-etal-2020-bart}(base) (denoising Transformer encoder-decoder)
    \item T5~\cite{colin-2020-T5}(base) (Transformer encoder-decoder)
    \item PEGASUS~\cite{zhang2020pegasus}
\end{itemize}
\subsubsection{Metrics}
\subsection{Results}\label{sec:results}

\begin{table}[tbh]\label{tab:home results}
\caption{Invidiual-level evaluation}
\center\setlength\tabcolsep{3.0pt}
\small
\begin{tabular}{|l|c|c|c|}
\hline
                     \multicolumn{4}{|c|}{\textbf{(a) Home \& Kitchen dataset}} \\
\hline
                     & \multicolumn{1}{c|}{Distinct-3} & \multicolumn{1}{c|}{BLEU} & \multicolumn{1}{c|}{METEOR} \\ \hline
MLE        & 7.77                                     & 18.13                              & 14.86                                \\ \hline
hMup        & 11.11                                    & 17.76                              & 15.40                                \\ \hline
% GAN-Utility &
% 12.96 & 15.20 & 12.82 \\ \hline
KPCNet      & 15.30                                    & 17.77                              & 16.18                                \\
\hline\hline
% GPT-2          & TBF                                    & TBF                             & TBF                      \\ \hline
BART %(3 epochs)       
& 11.04                                    & 19.15                             & 16.26                      \\ \hline
BART$_{DIV}$ %$_{d[0.1]}$ %(1 epoch)      
 & \ \ \ \ \ \ \ \ \ \ \ 17.10 \scriptsize{(+54.9\%)}                                    & \ \ \ \ \ \ \ \ \ 18.02 \scriptsize{(-6.3\%)}                             & \ \ \ \ \ \ \ \ \ 15.98 \scriptsize{(-1.8\%)}                  \\ \hline\hline
PEGASUS & 12.51 & 19.75 & \textbf{16.58} \\ \hline
PEGASUS$_{DIV}$ &\ \ \ \ \ \ \ \ \ \ \ \ \textbf{19.33} \scriptsize{(+54.5\%)} &\ \ \ \ \ \ \ \ \ 19.98 \scriptsize{(+1.2\%)} &\ \ \ \ \ \ \ \ 16.12 \scriptsize{(-2.9\%)} \\ \hline\hline
T5 %(3 epochs)   
& 14.28                                    & 19.24                              & 16.40                     \\ \hline
% T5 (5 epochs)         & 12.91                                    & 19.83                              & 16.27                       \\ \hline
T5$_{DIV}$%$_{d[0.05]}$ %(1 epoch) 
&\ \ \ \ \ \ \ \ \ \ \   17.53 \scriptsize{(+22.8\%)}                        &\ \ \ \ \ \ \ \ \ \ \textbf{20.10} \scriptsize{(+4.5\%)}                   &\ \ \ \ \ \ \ \ \ 16.32 \scriptsize{(-0.5\%)}                           \\ \hline

\multicolumn{4}{c}{} \\ \hline

                     \multicolumn{4}{|c|}{\textbf{(b) Office dataset}} \\
\hline

\hline
                     & \multicolumn{1}{c|}{Distinct-3} & \multicolumn{1}{c|}{BLEU} & \multicolumn{1}{c|}{METEOR} \\ \hline
MLE        & 20.33                                    & 14.73                              & 13.81                                \\ \hline
hMup        & 15.31                                    & 10.45                              & 12.52                                \\ \hline
KPCNet      & 30.99                                    & 13.84                              & 15.29                                \\ \hline\hline
BART %(10 epochs)    
& 31.74                                    & 10.43                              & 14.29    \\ \hline
BART$_{DIV}$%$_{d[0.05]}$ %(3 epochs)  
 & \ \ \ \ \ \ \ \ \ \ \ \textbf{40.11} \scriptsize{(+26.4\%)}   & \ \ \ \ \ \ \ \ \ \ \ 12.97  \scriptsize{(+24.4\%)}                          & \ \ \ \ \ \ \ \ \ 14.21 \scriptsize{(-0.5\%)}                   \\ \hline\hline
PEGASUS & 29.91 & 15.67 & 14.83 \\ \hline
PEGASUS$_{DIV}$ & \ \ \ \ \ \ \ \ \ \ \ 35.20 \scriptsize{(+17.7\%)} & \ \ \ \ \ \ \ \ \ 15.98 \scriptsize{(+2.0\%)} & \ \ \ \ \ \ \ \ \ 14.66 \scriptsize{(-1.2\%)} \\ \hline\hline
T5 %(3 epochs) 
& 24.40                                    & 16.76                              & 14.90                                \\ \hline
% T5 (5 epochs)         & 26.87                                    & 17.57                              & 14.93                                \\ \hline
T5$_{DIV}$%$_{d[0.1]}$ %(3 epochs) 
& \ \ \ \ \ \ \ \ \ \ \ 36.04 \scriptsize{(+47.7\%)}                        & \ \ \ \ \ \ \ \ \ \ \textbf{16.88} \scriptsize{(+1.3\%)}                            & \ \ \ \ \ \ \ \ \ \ \textbf{15.31}  \scriptsize{(+2.8\%)}                  \\ \hline

\end{tabular}
\end{table}


% \begin{table}[tbh]\label{tab:office results}
% \caption{Office dataset}
% \center\setlength\tabcolsep{3.0pt}
% \small
% \begin{tabular}{|l|c|c|c|}
% \hline
%                      & \multicolumn{1}{c|}{\textbf{Distinct-3}} & \multicolumn{1}{c|}{\textbf{BLEU}} & \multicolumn{1}{c|}{\textbf{METEOR}} \\ \hline
% MLE        & 20.33                                    & 14.73                              & 13.81                                \\ \hline
% hMup        & 15.31                                    & 10.45                              & 12.52                                \\ \hline
% KPCNet      & 30.99                                    & 13.84                              & 15.29                                \\ \hline\hline
% BART %(10 epochs)    
% & 31.74                                    & 10.43                              & 14.29    \\ \hline
% BART$_{DIV}$%$_{d[0.05]}$ %(3 epochs)  
%  & \ \ \ \ \ \ \ \ \ \ \textbf{40.11} \scriptsize{(+26.4\%)}   & \ \ \ \ \ \ \ \ \ \ 12.97  \scriptsize{(+24.4\%)}                          & \ \ \ \ \ \ \ \ 14.21 \scriptsize{(-0.5\%)}                   \\ \hline\hline
% PEGASUS & 29.91 & 15.67 & 14.83 \\ \hline
% PEGASUS$_{DIV}$ & \ \ \ \ \ \ \ \ \ \ 35.20 \scriptsize{(+17.7\%)} & \ \ \ \ \ \ \ \ \ 15.98 \scriptsize{(+2.0\%)} & \ \ \ \ \ \ \ \ 14.66 \scriptsize{(-1.2\%)} \\ \hline\hline
% T5 %(3 epochs) 
% & 24.40                                    & 16.76                              & 14.90                                \\ \hline
% % T5 (5 epochs)         & 26.87                                    & 17.57                              & 14.93                                \\ \hline
% T5$_{DIV}$%$_{d[0.1]}$ %(3 epochs) 
% & \ \ \ \ \ \ \ \ \ \ 36.04 \scriptsize{(+47.7\%)}                        & \ \ \ \ \ \ \ \ \ \textbf{16.88} \scriptsize{(+1.3\%)}                            & \ \ \ \ \ \ \ \ \ \textbf{15.31}  \scriptsize{(+2.8\%)}                  \\ \hline
% \end{tabular}
% \end{table}


\begin{table}[tbh]
\caption{Group-level evaluation (Home \& Kitchen)}
\small
\center\setlength\tabcolsep{3.0pt}
\begin{tabular}{|l|c|c|}
\hline
\multicolumn{1}{|l|}{} & \multicolumn{1}{c|}{\textbf{Avg-BLEU}} & \multicolumn{1}{c|}{\textbf{Pairwise-BLEU}} \\ \hline
MLE                    & 16.88                                  & 26.81\\ \hline
hMup                   & 9.88                                   & 13.38                                       \\ \hline
KPCNet                 & 16.19                                  & 42.81                                                       \\ \hline\hline
T5                     & 17.08                                  & 27.07                                       \\ \hline
T5$_{DIV}$                  & \ \ \ \ \ \ \ \ \ \ 17.24 \scriptsize{(+0.9\%)}                                 & \ \ \ \ \ \ \ \ \ \  26.21 \scriptsize{(+3.3\%)}                                       \\ \hline\hline
BART                   & 17.25                                  & 34.65                                       \\ \hline
BART$_{DIV}$                & \ \ \ \ \ \ \ \  \ 16.94  \scriptsize{(-1.8\%)}                                & \ \ \ \ \ \ \ \ \ 34.91  \scriptsize{(-0.7\%)}                                     \\ \hline\hline
PEGASUS                & 16.81                                  & 24.68                                       \\ \hline
PEGASUS$_{DIV}$           & \ \ \ \ \ \  \ \ \ \ 17.00  \scriptsize{(+1.1\%)}                                 & \ \ \ \ \ \ \ \ \ \ 23.84  \scriptsize{(+3.5\%)}                                     \\ \hline
\end{tabular}
\end{table}

  PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER
  PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER
  PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER
  PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER
  PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER
  PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER
  
  
    PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER
  PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER
  PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER
  PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER
  PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER
  PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER
  
  
    PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER
  PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER
  PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER
  PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER
  PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER
  PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER
  
    PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER
  PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER
  PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER
  PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER
  PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER
  PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER
